The Complexity of Equilibrium Refinements in Potential Games

The complexity of computing equilibrium refinements has been at the forefront of algorithmic game theory research, but it has remained open in the seminal class of potential games; we close this fundamental gap in this paper. We first show that computing a pure(-strategy) perfect or proper equilibrium is $\mathsf{PLS}$-complete in concise potential games in normal form. For pure perfect equilibria, we extend this result to general polytope games, which includes extensive-form games. We next turn to more structured classes of games, namely symmetric network congestion and symmetric matroid congestion games. For both classes, we show that a pure perfect equilibrium can be computed in polynomial time, strengthening the existing results for pure Nash equilibria. More broadly, we make a connection between strongly polynomial-time algorithms and efficient perturbed optimization using fractional interpolation. On the other hand, we establish that, for a certain class of potential games, there is an exponential separation in the length of the best-response path between perfect and Nash equilibria. Finally, for mixed strategies, we prove that computing a point geometrically near a perfect equilibrium requires a doubly exponentially small perturbation even in $3$-player potential games in normal form. As a byproduct, this significantly strengthens and simplifies a seminal result of Etessami and Yannakakis (FOCS '07). On the flip side, in the special case of polymatrix potential games, we show that equilibrium refinements are amenable to perturbed gradient descent dynamics, thereby belonging to the complexity class $\mathsf{CLS}$. This provides a principled and practical way of refining the landscape of gradient descent in constrained optimization.

==> figs/diagram.tex <==
\begin{tikzpicture}[
    node distance=1.5cm and 1.5cm,
    concept/.style={rectangle,draw,thick,minimum width=2cm,minimum height=1cm,align=center,fill=blue!3,font=\footnotesize},
    arrow/.style={-{latex},thick}
]

% Nodes
\node[concept] (nash) {Nash equilibria};
\node[concept,below=of nash] (subgame) {Subgame-perfect\\equilibria};
\node[concept,below=of subgame] (sequential) {Sequential\\equilibria};
\node[concept,below left=of sequential] (extensive) {Extensive-form\\perfect equilibria};
\node[concept,below right=of sequential] (quasi) {Quasi-perfect\\equilibria};
\node[concept,below=of quasi] (proper) {Normal-form\\proper equilibria};

% Arrows
\draw[arrow] (nash) -- (subgame);
\draw[arrow] (subgame) -- (sequential);
\draw[arrow] (sequential) -- (extensive);
\draw[arrow] (sequential) -- (quasi);
\draw[arrow] (quasi) -- (proper);

\end{tikzpicture}

==> figs/pennymatching.tex <==
\begin{tikzpicture}[
    scale=1.3,
    level distance=2cm,
    level 1/.style={sibling distance=6cm},
    level 2/.style={sibling distance=3cm},
    level 3/.style={sibling distance=1.5cm}
]

% Root node - Player 1
\node[circle,draw,line width=0.8pt,minimum size=7mm,fill=blue!12] (root) {$1$}
    child {
        node[circle,draw,line width=0.8pt,minimum size=7mm,fill=blue!12] (L1) {$1$}
        child {
            node[circle,draw,line width=0.8pt,minimum size=7mm,fill=red!12] (LL) {$2$}
            child {
                node[rectangle,draw,line width=0.6pt,minimum width=9mm,minimum height=5mm,font=\scriptsize] {$2,-2$}
                edge from parent node[left,draw=none,pos=0.3,font=\scriptsize] {\textsf{Heads}}
            }
            child {
                node[rectangle,draw,line width=0.6pt,minimum width=9mm,minimum height=5mm,font=\scriptsize] {$1,-1$}
                edge from parent node[right,draw=none,pos=0.3,font=\scriptsize] {\textsf{Tails}}
            }
            edge from parent node[left,draw=none,pos=0.3,font=\scriptsize] {\textsf{Gift}}
        }
        child {
            node[circle,draw,line width=0.8pt,minimum size=7mm,fill=red!12] (LR) {$2$}
            child {
                node[rectangle,draw,line width=0.6pt,minimum width=9mm,minimum height=5mm,font=\scriptsize] {$1,-1$}
                edge from parent node[left,draw=none,pos=0.3,font=\scriptsize] {\textsf{Heads}}
            }
            child {
                node[rectangle,draw,line width=0.6pt,minimum width=9mm,minimum height=5mm,font=\scriptsize] {$0,0$}
                edge from parent node[right,draw=none,pos=0.3,font=\scriptsize] {\textsf{Tails}}
            }
            edge from parent node[right,draw=none,pos=0.3,font=\scriptsize] {\textsf{NoGift}}
        }
        edge from parent node[left,draw=none,pos=0.25,font=\scriptsize, yshift=5pt] {\textsf{Heads}}
    }
    child {
        node[circle,draw,line width=0.8pt,minimum size=7mm,fill=blue!12] (R1) {$1$}
        child {
            node[circle,draw,line width=0.8pt,minimum size=7mm,fill=red!12] (RL) {$2$}
            child {
                node[rectangle,draw,line width=0.6pt,minimum width=9mm,minimum height=5mm,font=\scriptsize] {$1,-1$}
                edge from parent node[left,draw=none,pos=0.3,font=\scriptsize] {\textsf{Heads}}
            }
            child {
                node[rectangle,draw,line width=0.6pt,minimum width=9mm,minimum height=5mm,font=\scriptsize] {$2,-2$}
                edge from parent node[right,draw=none,pos=0.3,font=\scriptsize] {\textsf{Tails}}
            }
            edge from parent node[left,draw=none,pos=0.3,font=\scriptsize] {\textsf{Gift}}
        }
        child {
            node[circle,draw,line width=0.8pt,minimum size=7mm,fill=red!12] (RR) {$2$}
            child {
                node[rectangle,draw,line width=0.6pt,minimum width=9mm,minimum height=5mm,font=\scriptsize] {$0,0$}
                edge from parent node[left,draw=none,pos=0.3,font=\scriptsize] {\textsf{Heads}}
            }
            child {
                node[rectangle,draw,line width=0.6pt,minimum width=9mm,minimum height=5mm,font=\scriptsize] {$1,-1$}
                edge from parent node[right,draw=none,pos=0.3,font=\scriptsize] {\textsf{Tails}}
            }
            edge from parent node[right,draw=none,pos=0.3,font=\scriptsize] {\textsf{NoGift}}
        }
        edge from parent node[right,draw=none,pos=0.25,yshift=5pt, font=\scriptsize] {\textsf{Tails}}
    };

% Information sets for Player 2 (level 3)
% Connect nodes 1-3 (LL and RL)
\draw[line width=1.0pt,dashed,red!60] ($(LL)+(0,0.15)$) to[bend left=15] ($(RL)+(0,0.15)$);
% Connect nodes 2-4 (LR and RR)
\draw[line width=1.0pt,dashed,red!60] ($(LR)+(0,0.15)$) to[bend left=15] ($(RR)+(0,0.15)$);

\end{tikzpicture}

==> text/almostnear.tex <==







